A Decentralized Parallelization-in-Time Approach with Parareal

With steadily increasing parallelism for high-performance architectures, simulations requiring a good strong scalability are prone to be limited in scalability with standard spatial-decomposition strategies at a certain amount of parallel processors. This can be a show-stopper if the simulation results have to be computed with wallclock time restrictions (e.g.\,for weather forecasts) or as fast as possible (e.g. for urgent computing). Here, the time-dimension is the only one left for parallelization and we focus on Parareal as one particular parallelization-in-time method. We discuss a software approach for making Parareal parallelization transparent for application developers, hence allowing fast prototyping for Parareal. Further, we introduce a decentralized Parareal which results in autonomous simulation instances which only require communicating with the previous and next simulation instances, hence with strong locality for communication. This concept is evaluated by a prototypical solver for the rotational shallow-water equations which we use as a representative black-box solver.

==> 10_acknowledgements.tex <==
We are grateful to David Ham for the discussions on software design in general, to Stefan Zimmer for his valuable feedback on this work and to Alexander Breuer and Alexander Heinecke for their feedback on MPI progression.
We would also like to thank the University of Exeter for providing access to the Zen computer on which we computed the first benchmarks.
We would further like to thank the Munich Centre of Advanced Computing for supporting this project by providing computing time on the MAC Cluster.

==> 3_rswe.tex <==
%\label{sec:rswe}
%
%It is worth noting that Parareal methods have been
%successfully applied in the past
%%{\LARGE{(parallelised or just used in
%%    a serial simulation?) does it make a difference? :-) (Martin)} }
%to problems which are often dominated by
%dissipative stiffness (cf.\,\cite{Bal_Maday_02,Baffico_etal_02,Farhat_Chandesris_03,Garrido_etal_03}).
%The Parareal method was, however, not computationally feasible for
%weather and climate simulations until recently due to \textit{oscillatory stiffness.} 
%In this work we discuss parallelization of the
%\emph{asymptotic parallel-in-time method}\cite{Haut_Wingate_14}
%which permits the Parareal method to be applied to oscillatory-stiff
%problems.
%
%The approach used here for the coarse timestep uses both a longer timestep and a different physical model. Following the work of \cite{Embid_Majda_96} and \cite{Schochet_94}, the coarse solver uses a time homogenized version of the RSWE that is based on an asymptotic expansion \cite{Haut_Wingate_14}: 
%%and apply averaging with respect to some suitably-chosen smooth kernel over the fast waves.
%%Rewriting our problem in terms of an exponential integrator \cite{Cox_Matthews_02,Hochbruck_Ostermann_10}, we %may then pose the coarse problem, used for the coarse timestep, in the following form \cite{Haut_Wingate_14}:
%\begin{equation}
%\mathbf{u}(t) = e^{(-t/\epsilon)\mathcal{L}}\mathbf{\bar{u}}(t) + \mathcal{O}(\epsilon)
%\label{eq:apint_propagator}
%\end{equation}
%where the slowly varying function $\mathbf{\bar{u}}(t)$ satisfies the following reduced equation:
%\begin{equation} 
%\frac{\partial \mathbf{\bar{u}}}{\partial t} + \bar{\mathcal{N}}(\mathbf{\bar{u}},\mathbf{\bar{u}}) = \bar{\mathcal{D}}\mathbf{\bar{u}}
%\label{eq:slow_equation}
%\end{equation}
%Finally, the nonlinear and dissipative terms are given by the following time averages, performed with $\mathbf{\bar{u}}(t)$ held fixed:
%\begin{equation}
%\bar{\mathcal{N}}(\mathbf{\bar{u}}(t),\mathbf{\bar{u}}(t)) = \lim_{T \to \infty}\frac{1}{T}\int_{0}^{T}e^{s\mathcal{L}}\mathcal{N}(\mathbf{e^{-s\mathcal{L}}\bar{u}}(t),e^{-s\mathcal{L}}\mathbf{\bar{u}}(t))\,\mathrm{d}s
%\label{eq:nonlinear_averaged}
%\end{equation}
%\begin{equation}
%\bar{\mathcal{D}}(\mathbf{\bar{u}}(t)) = \lim_{T \to \infty}\frac{1}{T}\int_{0}^{T}(e^{s\mathcal{L}}\mathcal{D}\mathbf{e^{-s\mathcal{L}})\bar{u}}(t)\,\mathrm{d}s
%\label{eq:dissipative_averaged}
%\end{equation}
%In order to use this approximation for the coarse solver, we use a smooth kernel, $\rho(s)$, $0\le s \le 1$ which is chosen such that the length $T_{0}$ of the time window for the averaging is as small as possible, and approximate equation~[\ref{eq:nonlinear_averaged}] as:
%\begin{equation}
%\begin{aligned}
%\bar{\mathcal{N}}(\mathbf{\bar{u}}(t)) & \approx \frac{1}{T_{0}}\int_{0}^{T_{0}}\rho\left(\frac{s}{T_{0}}\right)e^{s\mathcal{L}}\mathcal{N}(e^{-s\mathcal{L}}\mathbf{\bar{u}}(t))\,\mathrm{d}s \\
%& \approx \frac{1}{\bar{M}}\sum\limits_{m=0}^{\bar{M}-1}\rho\left(\frac{s_{m}}{T_{0}}\right)e^{s_{m}\mathcal{L}}\mathcal{N}(e^{-s_{m}\mathcal{L}}\mathbf{\bar{u}}(t))
%\end{aligned}
%\end{equation}
%The above discretization of the long time averages can be interpreted as a variant of the Heterogeneous Multiscale Method (HMM) \cite{Engquist_Tsai_05}. The key point of using such a coarse solver is that all the time derivatives $\mathbf{u}(t)$ in equation (\ref{eq:slow_equation}) are formally independent of $ \epsilon$, and therefore a standard integrator may be used on (\ref{eq:slow_equation}) with large time steps $\Delta_T \gg \epsilon$. 
%
%In short, we use the averaged equations above for the coarse timestepping, while the fine timesteps involve the full solution of the PDE, using whichever method is preferred.
%
%\todo{Mention spectral method solvers here and that this method is used in results section}


==> 5_communication.tex <==
%\label{ref:communication}
%
%With MPI \cite{Forum:1994:MMI:898758} being the de-facto standard for parallelization on large-scale distributed systems, we focused on building up the Parareal simulation on this interface.
%For efficiency reasons, two important issues have to be considered:
%(1) The output of each coarse time interval has to be forwarded as fast as possible to the next coarse time interval,
%(2) The computation of the fine time stepping and hence also of the convergence via Parareal iteration has to be started as soon as possible.
%At first glance, it would appear that this could be accomplished by non-blocking send interfaces from the MPI.
%However, the MPI description only assures the required property (2): "A nonblocking
%send start call initiates the send operation, but does not complete it.
%The send start call can return before the message was copied out of the send buffer." \cite{Forum:1994:MMI:898758}.
%Here, it is not assured that the message is sent as fast as possible to the receiver as required by property (1).
%We refer the interested reader to \cite{hoefler2008message}.
%For the standard parallelization-in-space approach, this issue typically leads only to moderate performance drawbacks.
%However, for the Parareal parallelization-in-time approach this results in a major impact on the (parallel) performance, making the \emph{Parareal approach not applicable anymore} and even leads to an \emph{increase in wallclock time} -- independent of the number of additional cores.
%Therefore, we like to investigate this issue in the context of the Parareal approach in more depth.
%
%As soon as the domain resolution for our simulations was increased to $64^2$, we can observe a significant reduction in the Parareal performance.
%A detailed analysis shows a serialization of the communication, see Fig.\,\ref{fig:pypint_mpi_ctni0016_cores0016_res0064_shrinked}.
%Here, we can see a \emph{serialization of the communication} despite using non-blocking communication.
%Therefore, the entire Parareal algorithm is basically serialized and no performance speedup is gained.
%The wallclock time for running the simulation is even increased due to two overheads:
%the coarse time interval which has to be additionally computed without contributing to the final result and the communication overhead of communicating data to the next MPI ranks.
%
%\begin{figure}
%	\center
%	\includegraphics[width=0.45\textwidth]{pictures/pypint_mpi_ctni0016_cores0016_res0064_shrinked}
%	\caption{
%	Example of a serialized Parareal algorithm due to delayed sending of messages with a problem size of $64^2 \cdot 3 \cdot 8$ (3 quantities, double precision) with non-blocking communication:
%	The messages which are sent after the coarse time step (red bars) with a non-blocking send (isend) are not immediately sent to the next MPI rank.
%	Therefore, the coarse time step of the next coarse time step interval is executed only after the message is send and received.
%	Since this message is sent only after the fine time steps (blue bars), this leads to a \emph{serialization of the Parareal algorithm}.
%	}
%	\label{fig:pypint_mpi_ctni0016_cores0016_res0064_shrinked}
%\end{figure}
%
%We tested several variants to force sending of the message as soon as possible.
%Such results are MPI implementation specific and for this evaluation, we used IntelMPI.
%\begin{itemize}
%	\item Interleaving each fine timestep computation with an MPI Test:\newline
%		This did not result in any significant change in performance.
%
%	\item Two threads for sending and receiving:\newline
%		For the sender thread, the messages are stored in a queue and dequeued by the sender thread.
%		These messages are then sent with a blocking MPI ssend.
%		For the receiving thread, the messages are received and stored to a queue and dequeued by the main thread in case of requesting to receive a message.
%		This led to significant performance decreases.
%		We account for that by \emph{busy waiting} for receiving messages and hence resource conflicts due to pre-emptive scheduling.
%		Hence, the computing resource was not mainly used for simulations anymore, but also to wait for messages.
%	
%	\item Single sender thread:\newline
%		Using only a single sender thread avoided the aforementioned resource conflicts due to busy-waiting.
%		This led to the expected immediate sending behaviour.
%\end{itemize}
%
%The results in the next Section are based on the single sender thread implementation.


==> 6_performance_model.tex <==
%In this section, we present a performance model for a better understanding of the results.
%
%\begin{itemize}
%	\item $R$: Number of resources
%	\item $T_C$: Wallclock time for coarse time step
%	\item $T_F$: Wallclock time for fine time step
%	\item $T_x$: Wallclock time for data exchange
%	\item $C$: Number of coarse time steps
%\end{itemize}
%
%\subsection{Worst-case}
%The worst case is given by no convergence at all.
%Since this basically serializes the PinT algorithm, the runtime is even larger due to the additional computations for the coarse time step.
%
%The total runtime is then given by
%$$
%	T_{total} := (T_C + T_F + T_x) \cdot C
%$$
%, hence a speeddown of
%$$
%	S_{worst} := T_F \cdot C
%$$
%
%\subsection{Pint scalability limitation}
%To make the PinT algorithm performing well, obviously all computing resources are supposed to be involved in the computations.
%However, this is not possible if the coarse time propagator takes too much time. This induces severe idling time for two reasons:
%\begin{itemize}
%	\item The slices at the end of the sliding window are idling, since the latency is increased with a higher wall clocktime of coarse time steps.
%	\item Already converged slices at the beginning of the window are idling, since the solution still has to propagate through the system during initialization with the resources.
%\end{itemize}
%Hence, over a fixed period of simulation time and for an increasing number of resolution, the benefits of PinT vanish due to the above mentioned issues and the decreased convergence for the time slices at the end of the sliding window.
%
%TODO: model?!?


==> 8_conclusion.tex <==
\label{sec:conclusions}

% Interfaces
%We first presented a software approach for a realization of a Parareal controller.
%This approach hides the complexity of the Parareal approach and its requirement of MPI parallelization from the implementation of the problem to be solved parallel-in-time.
%Here, it is required that specific interfaces be implemented which we described in this work.
%Now, this allows fast prototyping of other ODE/PDE solvers with the Parareal method with the focus in this work on a PDE solver and with an MPI parallelization hidden from the developer.

% decentralized
%Second, we presented a decentralized realization of the Parareal method.
%With the Parareal method, only a communication from/to the previous/next coarse timestep interval is required.
%Our decentralized approach utilizes this locality by a state machine for each coarse time interval.
%Transitions of this state machine then only rely on locally triggered events or events triggered by the previous coarse time interval.
%By using a ring-communication, this directly results in an implementation of a so-called sliding window which is required in the case of restrictions on coarse timestep sizes.

% sender threads
%Third, we showed limitations of the MPI standard for Parareal regarding delayed sending of messages (see also \cite{hoefler2008message}).
%With a parallelization-in-space execution, such a delayed sending has only moderate impact on the parallel performance.
%However, for the Parareal method, we showed the importance of this issue which would directly lead to an increase of wallclock time, hence not allowing any scalability.
%We provided impact of this limitation by state plots, discussed and presented different solutions.
%For the MPI implementation used in this work, a single sender thread resulted in the best performance.

% Results
%We conducted several performance benchmarks based on a PDE solver used in a black-box way.
%This solver is based on a prototypical implementation of the rotational shallow-water equations.
%The Parareal method in combination with our decentralized approach leaves several space for future work:
%We expect, that an intercomparison with a variety of alternative approaches (e.g. based on tasks-parallelization on distributed memory systems) would show impact on locality-related effects and show limitations driven by memory movements and bandwidth limitations.
%This would allow adding and removing MPI ranks over the simulation runtime by inserting/removing coarse timestep intervals at/from the end of the sliding window.
%Therefore, we see a huge potential for dynamic resource management and the Parareal method to improve the resource utilization requirements among concurrently running applications.
%The decentralized approach can be used to avoid a single point-of-failure.
%This implicitly includes a huge potential to support fault tolerance in a way which is almost transparent to the application for upcoming Exascale architectures.


==> 9_terminology.tex <==
\todo{
	Add terminology, e.g.\,meaning of coarse time step size, coarse time interval, etc.
	Maybe also table of symbols.
}

